Case Study of Novelty, Complexity, and Adaptation in a Multicellular System

Continuing generation of novelty, complexity, and adaptation are well-established as core aspects of open-ended evolution. However, it has yet to be firmly established to what extent these phenomena are coupled and by what means they interact. In this work, we track the co-evolution of novelty, complexity, and adaptation in a case study from the DISHTINY simulation system, which is designed to study the evolution of digital multicellularity. In this case study, we describe ten qualitatively distinct multicellular morphologies, several of which exhibit asymmetrical growth and distinct life stages. We contextualize the evolutionary history of these morphologies with measurements of complexity and adaptation. Our case study suggests a loose -- sometimes divergent -- relationship can exist among novelty, complexity, and adaptation.

==> Makefile <==
SHELL=/bin/bash

# get the basename of the containing directory
# this will be used to name othe output document
BUILD_DIR := oee4



DRAFT_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}-draft.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

RELEASE_SUPPLEMENT_PAGE = $(shell pdftk ${BUILD_DIR}.pdf dump_data_utf8 | pcregrep -M -o1 '^BookmarkBegin\nBookmarkTitle: Supplemental Material\nBookmarkLevel: 1\nBookmarkPageNumber: ([0-9]+)$$')

all: ${BUILD_DIR}-draft.pdf

draft: ${BUILD_DIR}-draft.pdf ${BUILD_DIR}-manuscript-draft.pdf ${BUILD_DIR}-supplement-draft.pdf ${BUILD_DIR}-draft.tex

release: ${BUILD_DIR}.pdf ${BUILD_DIR}-manuscript.pdf ${BUILD_DIR}-supplement.pdf ${BUILD_DIR}.tex

${BUILD_DIR}.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR} \
    -pdflatex="pdflatex -interaction=nonstopmode" main.tex

${BUILD_DIR}.tex: main.tex
	./script/latexpand.pl main.tex > ${BUILD_DIR}.tex

${BUILD_DIR}-manuscript.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat 1-$$(( $(RELEASE_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript.pdf

${BUILD_DIR}-supplement.pdf: ${BUILD_DIR}.pdf
	pdftk ${BUILD_DIR}.pdf cat $(RELEASE_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement.pdf

${BUILD_DIR}-draft.pdf: main.tex
	latexmk -pdf -silent \
    -jobname=${BUILD_DIR}-draft \
    -pdflatex="pdflatex -interaction=nonstopmode" draft.tex

${BUILD_DIR}-draft.tex: main.tex
	./script/latexpand.pl draft.tex > ${BUILD_DIR}-draft.tex

${BUILD_DIR}-manuscript-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat 1-$$(( $(DRAFT_SUPPLEMENT_PAGE) - 1 )) output ${BUILD_DIR}-manuscript-draft.pdf

${BUILD_DIR}-supplement-draft.pdf: ${BUILD_DIR}-draft.pdf
	pdftk ${BUILD_DIR}-draft.pdf cat $(DRAFT_SUPPLEMENT_PAGE)-end output ${BUILD_DIR}-supplement-draft.pdf

fresh: cleaner all

clean:
	rm -f ${BUILD_DIR}.pdf
	rm -f ${BUILD_DIR}.tex
	rm -f ${BUILD_DIR}-draft.pdf
	rm -f ${BUILD_DIR}-draft.tex
	rm -f ${BUILD_DIR}-manuscript.pdf
	rm -f ${BUILD_DIR}-manuscript-draft.pdf
	rm -f ${BUILD_DIR}-supplement.pdf
	rm -f ${BUILD_DIR}-supplement-draft.pdf

sview:
	xdg-open ${BUILD_DIR}-draft.pdf 2>/dev/null

cleaner: clean
	latexmk -CA
	# remove auxillary files, excepting .tex and .bib files
	find . -type f -name ${BUILD_DIR}"*" ! -name '*.tex' ! -name '*.bib' -delete
	rm -rf *.bbl *.blg *.aux

.PHONY: draft release clean sview cleaner fresh


==> fig/cpu_detail.tex <==
\begin{figure}

\includegraphics[width=\linewidth]{{img/cpu_detail}}

\caption{
\textbf{Overview of genome execution.}
\footnotesize
Tagged events and messages (shown as bells and envelopes, respectively) activate module execution on virtual cores.
Simulation state can also be read directly using sensor instructions to access input registers.
Special instructions write to output registers, allowing interaction with the simulation, and generate tagged messages, allowing interaction with other virtual CPUs.
}
\label{fig:cpu_detail}
\end{figure}


==> fig/fitness.tex <==
\begin{figure}

\input{fig/fitness/fitness_neutrality.tex}
\input{fig/fitness/fitness_magnitude.tex}
\input{fig/fitness/doubling_time.tex}

\caption{ Fitness assays.
Color coding and letters correspond to qualitative morph codes described in Table \ref{tab:morph_descriptions}.
Dotted vertical line denotes emergence of morph $e$.
Dashed vertical line denotes emergence of morph $g$. }
\label{fig:fitness}

\end{figure}


==> fig/fitness/doubling_time.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/fitness/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-vline+x=stint+y=mean-doubling-time-growth-rate+ext=}}

\caption{Growth rate estimated from doubling time experiments, measuring time for a monoculture to grow from 0.25 maximum population size to 0.5 maximum population size.}
\label{fig:fitness:doubling_time}

\end{subfigure}%


==> fig/fitness/fitness_magnitude.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/fitness/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-vline-hline+x=stint+y=median-fitness-differential-against-immediate-predecessor-population+ext=}}

\caption{Magnitude of fitness differential against immediately-preceding stint population.
Positive fitness differential indicates greater fitness compared to predecessor.
Solid horizontal line indicates neutral fitness differential.
}
\label{fig:fitness:fitness_magnitude}

\end{subfigure}%


==> fig/fitness/fitness_neutrality.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/fitness/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-vline-binomialh0+x=stint+y=fraction-immediate-predecessor-battles-won+ext=}}

\caption{
Fraction of 20 independent competitions that were won against immediate predecessor population.
Blue horiziontal lines represent significance level $p < 0.05$ for binomial null hypothesis.
Neutral outcomes fall inside the blue bars, significant fitness increases fall above them, and significant fitness decreases fall below them.
}
\label{fig:fitness:fitness_neutrality}

\end{subfigure}%


==> fig/fitness_complexity.tex <==
\begin{figure}

\input{fig/fitness_complexity/critical_fitness_complexity.tex}
% \input{fig/fitness_complexity/interpolated_fitness_complexity.tex}
% \input{fig/fitness_complexity/composite_fitness_complexity.tex}

\caption{ Fitness complexity estimates. Color coding and letters correspond to qualitative morph codes described in Table \ref{tab:morph_descriptions}.
Dotted vertical line denotes emergence of morph $e$.
Dashed vertical line denotes emergence of morph $g$.
}
\label{fig:fitness_complexity}

\end{figure}


==> fig/fitness_complexity/composite_fitness_complexity.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/composite_fitness_complexity/bucket=prq49+cat=morph+ci=95+endeavor=16+transform=filter-Series-16005+viz=letterscatter-err-vline+x=stint+y=composite-fitness-complexity+ext=}}

\caption{
Composite fitness complexity.
Sum of critical fitness complexity and interpolated fitness complexity.
Error bars represent 95\% credible interval.
Vertical gray bars represent missing estimates due to bad phenotype-neutral nopouts.
Supplementary Figure \ref{fig:fitness_complexity_alt:composite_fitness_complexity_alt} shows the same data with smaller markers.
}
\label{fig:fitness_complexity:composite_fitness_complexity}

\end{subfigure}%


==> fig/fitness_complexity/critical_fitness_complexity.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/critical_fitness_complexity/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-vline+x=stint+y=critical-fitness-complexity+ext=}}

\caption{
Critical fitness complexity.
Number of single-site nopouts that significantly decrease fitness, adjusted for expected false positives.
}
\label{fig:fitness_complexity:critical_fitness_complexity}

\end{subfigure}%


==> fig/fitness_complexity/interpolated_fitness_complexity.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/interpolated_fitness_complexity/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-err-vline+x=stint+y=interpolated-fitness-complexity+ext=.pdf}}

\caption{Interpolated fitness complexity.
Estimated number of non-critical sites that contribute to fitness.
Vertical gray lines represent stints with missing estimates due to bad phenotype-neutral nopouts.
Shaded areas represent 95\% confidence intervals.
Supplementary Figure \ref{fig:fitness_complexity_alt:interpolated_fitness_complexity_alt} shows the same data with smaller markers.
}
\label{fig:fitness_complexity:interpolated_fitness_complexity}

\end{subfigure}%


==> fig/fitness_complexity_alt.tex <==
\begin{figure}

% \input{fig/fitness_complexity_alt/composite_fitness_complexity_alt.tex}
% \input{fig/fitness_complexity_alt/interpolated_fitness_complexity_alt.tex}

\caption{
Stub of content removed from supplement.
Left in to maintain figure numbering.
% Alternate renderings of Figure \ref{fig:fitness_complexity}.
}
\label{fig:fitness_complexity_alt}

\end{figure}


==> fig/fitness_complexity_alt/composite_fitness_complexity_alt.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/composite_fitness_complexity_alt/bucket=prq49+ci=95+endeavor=16+transform=filter-Series-16005+viz=scatter-err-vline+x=stint+y=composite-fitness-complexity+ext=}}

\caption{ Composite fitness complexity.
% An alternate rendering of Figure \ref{fig:fitness_complexity:composite_fitness_complexity}.
}
\label{fig:fitness_complexity_alt:composite_fitness_complexity_alt}

\end{subfigure}%


==> fig/fitness_complexity_alt/interpolated_fitness_complexity_alt.tex <==
\begin{subfigure}{0.5\textwidth}

\includegraphics[width=\linewidth]{{plots/interpolated_fitness_complexity_alt/bucket=prq49+endeavor=16+transform=filter-Series-16005+viz=scatter-err-vline+x=stint+y=interpolated-fitness-complexity+ext=}}

\caption{ Interpolated fitness complexity.
% An alternate rendering of Figure \ref{fig:fitness_complexity:interpolated_fitness_complexity}.
}
\label{fig:fitness_complexity_alt:interpolated_fitness_complexity_alt}

\end{subfigure}%


==> fig/phenotype_complexity.tex <==
\begin{figure}

\includegraphics[width=\linewidth]{{plots/phenotype_complexity/bucket=prq49+cat=morph+endeavor=16+transform=filter-Series-16005+viz=letterscatter-vline+x=stint+y=phenotype-complexity+ext=}}

\caption{ Number of genome sites that contribute to phenotpe, measured as number sites remaining after phenotype-neutral nopout.
Color coding and letters correspond to qualitative morph codes described in Table \ref{tab:morph_descriptions}.
Dotted vertical line denotes emergence of morph $e$.
Dashed vertical line denotes emergence of morph $g$.
}
\label{fig:phenotype_complexity}
\end{figure}


==> fig/phylo_nj_tree.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{{submodule/dishtiny_event_tag_phylogenetics/teeplots/phylo_tree_no_outliers/viz=draw+ext=}}

\caption{
Phylogeny of sampled focal strain representatives across stints reconstructed using neighbor-joining algorithm \citep{cock2009biopython}.
Each leaf node corresponds to a sampled representative.
Representatives from stints 0 and 1, which share no common ancestry with representatives from other stints, are excluded.
Numbers refer to stint that each representative was sampled from.
Color coding and parentheticals of stint labels correspond to qualitative morph codes described in Table \ref{tab:morph_descriptions}.
}
\label{fig:phylo_nj_tree}
\end{figure*}


==> fig/phylo_scipy_linkage_tree.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{{submodule/dishtiny_event_tag_phylogenetics/teeplots/scipy_linkage_tree_no_outliers/viz=draw+ext=}}

\caption{
Phylogeny of sampled focal strain representatives across stints reconstructed using hierarchical clustering algorithm \citep{virtanen2020scipy}.
Each leaf node corresponds to a sampled representative.
Representatives from stints 0 and 1, which share no common ancestry with representatives from other stints, are excluded.
Numbers refer to stint that each representative was sampled from.
Color coding and parentheticals of stint labels correspond to qualitative morph codes described in Table \ref{tab:morph_descriptions}.
}
\label{fig:phylo_scipy_linkage_tree}
\end{figure*}


==> lib/importpath.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/17491
\makeatletter
  \providecommand\importpath{\import@path}
\makeatother


==> lib/replacesinglequote.tex <==
\pragmaonce

% adapted from https://tex.stackexchange.com/a/8620
\def\replacesinglequote#1{%
  \IfSubStr{#1}{'}{%
    \StrSubstitute{#1}{'}{\,}}{#1}}


==> lib/safepercent.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/351125
\catcode`\%=12
\providecommand\safepercent{%}
\catcode`\%=14


==> lib/safetilde.tex <==
% \pragmaonce

% adapted from https://tex.stackexchange.com/a/425957
\providecommand\safetilde{\string~}


==> listing/probability_deleterious.tex <==
\begin{lstlisting}[language=python, caption={Formula to calculate probability of deleterious outcome in nopout interpolation.}, label={lst:probability_deleterious}]
import math

def count_hands_with_k_or_more_sets(
    deck_size, hand_size, num_sets, set_size, k
):

    num_fixed = set_size * k
    deck_free = deck_size - num_fixed
    hand_free = hand_size - num_fixed

    if k > num_sets or k > hand_size or deck_free < 0 or hand_free < 0:
        return 0

    if set_size == 1:
        return sum(
            math.comb(num_sets, k_)
            * math.comb(deck_size - num_sets, hand_size - k_)
            for k_ in range(k, num_sets + 1)
            if hand_size >= k_
        )

    return (
        math.comb(deck_free, hand_free)
        * math.comb(num_sets, k)
    ) - count_hands_with_k_or_more_sets(
        deck_size,
        hand_size,
        num_sets,
        set_size,
        k=k+1,
    )

def probability_deleterious(
    n, h, m, s
):
    return count_hands_with_k_or_more_sets(
        n, h, m, s, 1
    ) / math.comb(n, h)

\end{lstlisting}

